Onomastics 2.0 - The Power of Social Co-Occurrences

Onomastics is "the science or study of the origin and forms of proper names of persons or places." ["Onomastics". Merriam-Webster.com, 2013. http://www.merriam-webster.com (11 February 2013)]. Especially personal names play an important role in daily life, as all over the world future parents are facing the task of finding a suitable given name for their child. This choice is influenced by different factors, such as the social context, language, cultural background and, in particular, personal taste. With the rise of the Social Web and its applications, users more and more interact digitally and participate in the creation of heterogeneous, distributed, collaborative data collections. These sources of data also reflect current and new naming trends as well as new emerging interrelations among names. The present work shows, how basic approaches from the field of social network analysis and information retrieval can be applied for discovering relations among names, thus extending Onomastics by data mining techniques. The considered approach starts with building co-occurrence graphs relative to data from the Social Web, respectively for given names and city names. As a main result, correlations between semantically grounded similarities among names (e.g., geographical distance for city names) and structural graph based similarities are observed. The discovered relations among given names are the foundation of "nameling" [http://nameling.net], a search engine and academic research platform for given names which attracted more than 30,000 users within four months, underpinningthe relevance of the proposed methodology.

==> application.tex <==
%------------------------------------------------------------------------------
\section{Application}\label{sec:application}
%------------------------------------------------------------------------------
%------------------------------------------------------------------------------
\begin{figure}
  \centering
  \includegraphics[width=0.3\linewidth]{results/category_prediction/cosine-weiblich}
  \includegraphics[width=0.3\linewidth]{results/category_prediction/cosine-maennlich}
  \includegraphics[width=0.3\linewidth]{results/category_prediction/cosine-tuerkisch}

  \caption{Category precision for gender.}
  \label{fig:similarities:categoryprediction}
\end{figure}
%------------------------------------------------------------------------------

